Grammatical Error Correction with Neural Reinforcement Learning

We propose a neural encoder-decoder model with reinforcement learning (NRL) for grammatical error correction (GEC). Unlike conventional maximum likelihood estimation (MLE), the model directly optimizes towards an objective that considers a sentence-level, task-specific evaluation metric, avoiding the exposure bias issue in MLE. We demonstrate that NRL outperforms MLE both in human and automated evaluation metrics, achieving the state-of-the-art on a fluency-oriented GEC corpus.

==> related.tex <==
\section{Related Work}
\begin{itemize}
\item Direct optimization has recently been applied to \proposed for MT. 
\item Reinforcement learning becomes prominent in Dialogue.
\end{itemize}
